Game-theoretic Counterfactual Explanation for Graph Neural Networks

Graph Neural Networks (GNNs) have been a powerful tool for node classification tasks in complex networks. However, their decision-making processes remain a black-box to users, making it challenging to understand the reasoning behind their predictions. Counterfactual explanations (CFE) have shown promise in enhancing the interpretability of machine learning models. Prior approaches to compute CFE for GNNS often are learning-based approaches that require training additional graphs. In this paper, we propose a semivalue-based, non-learning approach to generate CFE for node classification tasks, eliminating the need for any additional training. Our results reveals that computing Banzhaf values requires lower sample complexity in identifying the counterfactual explanations compared to other popular methods such as computing Shapley values. Our empirical evidence indicates computing Banzhaf values can achieve up to a fourfold speed up compared to Shapley values. We also design a thresholding method for computing Banzhaf values and show theoretical and empirical results on its robustness in noisy environments, making it superior to Shapley values. Furthermore, the thresholded Banzhaf values are shown to enhance efficiency without compromising the quality (i.e., fidelity) in the explanations in three popular graph datasets.

==> Other/README.tex <==
\section{\textcolor{red}{README}}



\textcolor{red}{NOT PART OF THE DOCUMENT}. This section is for tracking the work in progress.

\subsection{Project Tasks}

\subsubsection{Experimental Results}
\begin{enumerate}
    \vspace{-0.7em}\item Baseline: Greedy
    \vspace{-0.7em}\item Baseline: Naive top-k (selected individually)
    \vspace{-0.7em}\item Baseline: Brute-force search all combinations (very slow)
    
    \vspace{0.5em}\item GT approach: Shapley Value
    \vspace{-0.7em}\item GT approach: Banzahf Power Index
    \vspace{-0.7em}\item GT approach: Core 
    \vspace{-0.7em}\item GT approach: Shapley–Shubik power index (very low-priority, looks like it is easy)
    
\end{enumerate}


\subsubsection{Theoretical Results}
\begin{enumerate}
    \vspace{-0.7em}\item Guarantees for Sampling while calculating values
    \vspace{-0.7em}\item Explanations mostly being in the neighborhood of the node.
\end{enumerate}

\subsubsection{Misc. Tasks}
\begin{enumerate}
    \vspace{-0.7em}\item Faster edge deletion.
    \vspace{-0.7em}\item Proper handling of undirected graphs.
\end{enumerate}


\subsection{Other Ideas}
\begin{enumerate}
    \vspace{-0.7em}\item Better sampling techniques than random
    \vspace{-0.7em}\item Highly connected explanations being better than sparse ones.
\end{enumerate}

\subsection{Priority}

The following two tasks makes future work a lot easier.

\begin{enumerate}
    \item Optimization 1: Using masks on the GNN to get the probability changes. Currently we are doing full deletions and additions. Iterating through the tensor is super slow.
    \item Optimization 2: Sampling elements from the powerset without enumerating the whole set first. (Non trivial when we don't want repeating elements)
    \item Main paper: \url{https://proceedings.mlr.press/v206/wang23e/wang23e.pdf}
\end{enumerate}

\subsection{Things to do}
\begin{enumerate}
    \item Optimizations \sm{List them down} \sj{The optimizations are listed above in section 1.3, I have solved both the optimizations. Both the optimizations are for the Shapley value using Hersanyi dividend }
    \item Other methods (banzhaf and core) \sm{what about their optimizations?}
    \item Other datasets (like PolBlogs) \sm{Be concrete - list them down} \sj{Working on it, will add them soon}
    \item Bigger hop size \sm{This is a robustness check - you have to find other hyperparameters as well}
    \item Other approximation methods (for Shapley) \sm{What are they exactly} \sj{Working on it, will add them soon}
    \item Other Tasks (Graph Classification)
\end{enumerate}

==> Other/meeting_notes.tex <==
\section{Meeting Notes}

\subsection{29th June, 2023}
% just add bullet points about what we discussed and next steps and if there are any big ideas.
Discussion:
\begin{itemize}
    \item Problem definition: Explain node classification by assigning feature importance to edges. Feature importance is calculated using various approaches: Greedy cut, Shapley value, or selecting the top k edges.(Feature importance is being measured using the fidelity metric) \item Issues to investigate:
    \begin{itemize}
        \item Which edges to consider for deletion: within 1 hop, 2 hop or more? For now, consider only till 2 hops.
        \item How to cleverly sample edges for calculating shapley value?
    \end{itemize} 
\end{itemize}

Next steps:
\begin{itemize}
    \item Implement shapley value
    \item Try to correlate Shapley value properties with our problem so as to provide a justification of why we use a particular game theoretic approach 
\end{itemize}

\subsection{Aug 22 2023}
Points discussed:
\begin{itemize}
    \item Change the current way of calculating the fidelity metric: calculate it as the standard metric in which the lower value is better
    \item Concretize the experiment design: finalize the datasets, the metrics to be used, the hyperparameters and their values to be tuned, the other algorithms against which the results need to be compared
    \item Make shapely value implementation faster
    \item Implement BI
    \item Try to come up with theoretical results regarding the approximations of shapely value (Coalition size and the size of a coalition)
\end{itemize}
